The Value, Benefits, and Concerns of Generative AI-Powered Assistance in Writing

Recent advances in generative AI technologies like large language models raise both excitement and concerns about the future of human-AI co-creation in writing. To unpack people's attitude towards and experience with generative AI-powered writing assistants, in this paper, we conduct an experiment to understand whether and how much value people attach to AI assistance, and how the incorporation of AI assistance in writing workflows changes people's writing perceptions and performance. Our results suggest that people are willing to forgo financial payments to receive writing assistance from AI, especially if AI can provide direct content generation assistance and the writing task is highly creative. Generative AI-powered assistance is found to offer benefits in increasing people's productivity and confidence in writing. However, direct content generation assistance offered by AI also comes with risks, including decreasing people's sense of accountability and diversity in writing. We conclude by discussing the implications of our findings.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> chickenribs.tex <==
% To promote more appropriate reliance on AI assistants, researchers have attempted different approaches and achieved a certain degree of success, such as enhancing the model transparency \cite{wang2021explanations, poursabzi2021manipulating, kaur2020interpreting, yang2020visual, adadi2018peeking, liu2021understanding, mitchell2019model}, letting users understand the limitations of AI assistants \cite{chiang2021you, ashktorab2021ai}, nudging people to rethink the decision \cite{buccinca2021trust}, and improving people's AI literacy \cite{zimmerman2018teaching, long2020ai, chiang2022exploring}. 

% The biased decision can be contributed by the AI assistants' bias \cite{buolamwini2018gender, mehrabi2021survey, de2019bias} or people's bias toward the AI assistant \cite{green2019principles, green2019disparate}.




% COMPAS model is notorious for its racial discrimination, which overrates the risk on Black defendants and underrates the risk of White defendants despite the similar accuracy. Interestingly, our results show that the people in groups rely on the model more than the individuals. At first glance, the finding contradicts the intuition. However, a further analysis indicates that people in groups rely on the model more on Black defendants than on White defendants ($\Delta$REL>0), while individuals do the opposite way ($\Delta$REL<0).  


% Previous research shows that human predictions tend to overestimate the recidivism risk and hence was less accurate than the COMPAS \cite{tan2018investigating}. Similar to \cite{tan2018investigating}, the responses in Phase 1 also show that people, compared to COMPAS, overestimated the recidivism risk of defendants \cc{add data.} Due to COMPAS underestimate the risk of White defendants, 
% , which is similar to the findings without AI involvement \cite{wright1996impact, kerr1996bias}.
% \cc{For example, compared to individuals, groups tend to attenuate unsystematic, random errors (see Page Shapiro, 1992; Zajonc, 1962)}



% \cc{Comminucation: cites ``Individual performance in team-based online games'' }
% \cc{public don't understand the fairness measures cites: ``Measuring Non-Expert Comprehension of Machine Learning Fairness Metrics''}
% \cc{ We speculate that this observation may be related to arguments from recent studies that group membership reduces the sense of responsibility and regret that members may face under the same circumstances individually. If correct, a reduced emotional barrier to action may be an underlying mechanism driving group members to act earlier. cite: M. El Zein, B. Bahrami, R. Hertwig, Shared responsibility in collective decisions. Nat. Hum. Behav. 3, 554–559 (2019).}



% The results suggested no significant difference in the subject's confidence between conditions when she agreed with the model suggestion (p = 0.732). However, subjects adopting collective decisions were more confident in their final decision than subjects who did not, when they suspected and did not follow the model suggestions (p = 0.003).

% Anchoring effect, people's opinions would be affected by the first provided opinion \cite{strack1997explaining}, could not fully explain the phenomenon because both treatments received the AI suggestions before making the prediction. If the anchoring effect exists in our experiment, it will lead both treatments to rely on the model but not make the differences between the two treatments. 
% Yet, Bandwagon effect, people who do not have strong opinions tend to follow the mainstream point of view \cite{van2016off}, might explain the reliance difference. From the group discussion in our experiment, we also observed the existence of the Bandwagon effect leading people to rely on AI suggestions especially when the people cannot reach a consensus and do not have strong preferences:



% Then, we computed the cosine similarity between each member's potential feature preference and defined the cognitive diversity score of a group as the negative of the maximum potential feature preference similarity among members in the group.
% In other words, group diversity is how different the most similar members are in the group, and the diversity score between any two members in the group is greater than the group diversity score. The diversity score ranges from -1 to 1, where -1 represents that at least two members in the group have the same viewpoint on the recidivism risk task, and 1 means that all members have entirely opposite opinions on the recidivism risk task (i.e., in a two-member group, one member considers White defendants are more likely reoffend, but another member considers Black defendants are more likely reoffend). If the diversity score is 0, it indicates all members consider the different features to play the most critical roles in the recidivism risk task; for instance, one member feels the race of the defendants is the only reason that impact the defendant's reoffend risk, but another member thinks the charge degree is the only reason of it. 


% To understand the impact of cognitive diversity, we first split the subject entity in the Group-AI condition into a heterogeneous group if its diversity score is greater than 0 and the homogeneous group otherwise.



% AI-driven decision aids have been widely used to assist people in making important decisions and achieve different levels of success in diverse domains, such as criminal sentences \cite{larson2016we}, financial investment \cite{tsaih1998forecasting}, and medical diagnosis \cite{esteva2017dermatologist, cai2019hello}. In these AI-assisted decision-making settings, AI models provide suggestions to people so that they can utilize the suggestions and make their final decisions. For instance, in the healthcare area, AI systems are being developed to provide the initial disease detection to a team of physicians, and the team has to evaluate the detection and further determine the further treatment \cite{cai2019hello}.\zl{better to use an individual example here} With the rapid growth of decision aids that AI models drive, research on understanding whether and how individuals use the AI assistant in decision-making has recently been widely explored \cite{amershi2019guidelines, dietvorst2015algorithm, chong2022human, poursabzi2021manipulating, gemalmaz2022understanding}.
% For instance, AI systems are being developed to give the probe medical diagnosis to the physician, and hence physician has to evaluate the advice and further determine the treatment \cite{cai2019hello}.\zl{maybe remove this example?} 


% Throughout history, most human achievements have been developed by team collaborations, not alone by individuals. In practical AI-assisted decision-making settings, people work with others and make decisions collectively. In the health care example, \cite{cai2019hello}, the final decision of whether to adopt the AI's initial detection is not made by a single individual but by a group of people. In collective decision-making, an individual's opinion may be adapted or inspired by other group members' opinions \cite{dalkey1969delphi}. Hence, the human behaviors observed in the individual setting could not directly apply to the group collaboration setting. However, our knowledge of whether and how collective decision-making changes people's behavior with and perception of AI assistants in decision-making is largely limited.
